Data-Driven Debugging for Functional Side Channels

Information leaks through side channels are a pervasive problem, even in security-critical applications. Functional side channels arise when an attacker knows that a secret value of a server stays fixed for a certain time. Then, the attacker can observe the server executions on a sequence of different public inputs, each paired with the same secret input. Thus for each secret, the attacker observes a function from public inputs to execution time, for instance, and she can compare these functions for different secrets. First, we introduce a notion of noninterference for functional side channels. We focus on the case of noisy observations, where we demonstrate with examples that there is a practical functional side channel in programs that would be deemed information-leak-free or be underestimated using the standard definition. Second, we develop a framework and techniques for debugging programs for functional side channels. We extend evolutionary fuzzing techniques to generate inputs that exploit functional dependencies of response times on public inputs. We adapt existing results and algorithms in functional data analysis to model the functions and discover the existence of side channels. We use a functional extension of standard decision tree learning to pinpoint the code fragments causing a side channel if there is one. We empirically evaluate the performance of our tool FUCHSIA on a series of micro-benchmarks and realistic Java programs. On the set of benchmarks, we show that FUCHSIA outperforms the state-of-the-art techniques in detecting side channel classes. On the realistic programs, we show the scalability of FUCHSIA in analyzing functional side channels in Java programs with thousands of methods. Also, we show the usefulness of FUCHSIA in finding side channels including a zero-day vulnerability in OpenJDK and another vulnerability in Jetty that was since fixed by the developers.

==> Makefile <==
# NOTE: you must install latexmk first!!

LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

MAIN=main
SOURCES=$(MAIN).tex Makefile introduction.tex overview.tex motivation.tex definition.tex discovery.tex overallAlg.tex impDtl.tex environment.tex experiment.tex case-study.tex related.tex conclusion.tex  header.tex papers.bib regex-code.tex regex-flow.tex jetty-code.tex jetty-flow.tex motivation_figures_1.tex motivation_figures.tex case-study-figs-1.tex case-study-figs-2.tex case-study-figs-3.tex case-study-figs-4.tex experiment-table.tex threat-validity.tex apps-micro-benchmark.tex ack.tex
FIGURES=
#FIGURES := $(shell find figures/* images/* -type f)

all:    $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) \
	-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

online: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk *.refresh *.DS_Store

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all


==> case-study-figs-3.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.25\textwidth]{Figures/apache_ftp_cost_bytecode.png}
  %\includegraphics[width=0.3\textwidth]{Figures/Jetty_clustered.png}
  \hfill
  \scalebox{0.4}{
    \begin{tikzpicture}[align=center,node distance=1cm,->,thick,
        draw = black!60, fill=black!60]
      \centering
      \pgfsetarrowsend{latex}
      \pgfsetlinewidth{0.3ex}
      \pgfpathmoveto{\pgfpointorigin}


      \node[dtreenode,initial above,initial text={}] at (0,0) (l0)  {
        org...usermanager.SaltedPassword\\Encryptor.regionMatches\_bblock\_121};
      \node[dtreenode,below=of l0] (l2)
       {org...usermanager.SaltedPassword\\Encryptor.regionMatches\_bblock\_121};
       \node[dtreenode,below=of l2] (l4)
        {org...usermanager.SaltedPassword\\Encryptor.regionMatches\_bblock\_121};
        \node[below=of l4] (l6) {};

        \node[dtreeleaf,bicolor={black and black and 0.99},below left=of
          l0] (l1) {};
        \node[dtreeleaf,bicolor={red and red and 0.99},below left=of l2]
        (l3) {};
        \node[dtreeleaf,bicolor={green and green and 0.99},below left=of
          l4] (l5) {};

        \path[->]  (l0) edge  node [left,pos=0.4] {$ = \beta_1 ~~$} (l1);
        \path  (l0) edge  node [right, pos=0.4] {$~~ \neq \beta_1 $} (l2);
        \path  (l2) edge  node [left] {$ = \beta_2 ~~$} (l3);
        \path  (l2) edge  node [right] {$~~ \neq \beta_2 $} (l4);
        \path  (l4) edge  node [left] {$ = \beta_3 ~~$} (l5);
        \path  (l4) edge[dotted]  node [right] {$~~ \neq \beta_3$} (l6);
    \end{tikzpicture}
  }
	\hfill
	\includegraphics[width=0.25\textwidth]{Figures/authmreloaded_cost.png}
  %\includegraphics[width=0.3\textwidth]{Figures/Jetty_clustered.png}
  \hfill
  \scalebox{0.4}{
    \begin{tikzpicture}[align=center,node distance=1cm,->,thick,
        draw = black!60, fill=black!60]
      \centering
      \pgfsetarrowsend{latex}
      \pgfsetlinewidth{0.3ex}
      \pgfpathmoveto{\pgfpointorigin}


      \node[dtreenode,initial above,initial text={}] at (0,0) (l0)  {
        fr.xephi.authme.security.crypts\\UnsaltedMethod.isEqual\_bblock\_66};
      \node[dtreenode,below=of l0] (l2)
       {fr.xephi.authme.security.crypts\\UnsaltedMethod.isEqual\_bblock\_66};
       \node[dtreenode,below=of l2] (l4)
        {fr.xephi.authme.security.crypts\\UnsaltedMethod.isEqual\_bblock\_66};
        \node[below=of l4] (l6) {};

        \node[dtreeleaf,bicolor={green and green and 0.99},below left=of
          l0] (l1) {};
        \node[dtreeleaf,bicolor={red and red and 0.99},below left=of l2]
        (l3) {};
        \node[dtreeleaf,bicolor={blue and blue and 0.99},below left=of
          l4] (l5) {};

        \path[->]  (l0) edge  node [left,pos=0.4] {$ = \beta_1 ~~$} (l1);
        \path  (l0) edge  node [right, pos=0.4] {$~~ \neq \beta_1 $} (l2);
        \path  (l2) edge  node [left] {$ = \beta_2 ~~$} (l3);
        \path  (l2) edge  node [right] {$~~ \neq \beta_2 $} (l4);
        \path  (l4) edge  node [left] {$ = \beta_3 ~~$} (l5);
        \path  (l4) edge[dotted]  node [right] {$~~ \neq \beta_3$} (l6);
    \end{tikzpicture}
  }

	\hfill
	\caption{
		(a) Apache FTP Server timing functions.
		(b)	Apache FTP Server explanations.
		(c) Github Authmreloaded timing functions.
		(d) Github Authmreloaded explanations.
	}
	\label{fig:apache-ftp-clustered}
	\label{fig:apache-ftp-DT}
	\label{fig:github-clustered}
	\label{fig:github-DT}
	\vspace{-1.0em}
\end{figure*}


==> jetty-flow.tex <==
\begin{figure*}[t!]
  \centering
  %\includegraphics[width=0.3\textwidth]{Figures/Jetty_initial.png}
  \includegraphics[width=0.27\textwidth]{Figures/Jetty_remote.png}
  \hfill
  \includegraphics[width=0.27\textwidth]{Figures/Jetty_match.png}
  %\includegraphics[width=0.3\textwidth]{Figures/Jetty_clustered.png}
  \hfill
  \scalebox{0.55}{
    \begin{tikzpicture}[align=center,node distance=1cm,->,thick,
        draw = black!60, fill=black!60]
      \centering
      \pgfsetarrowsend{latex}
      \pgfsetlinewidth{0.3ex}
      \pgfpathmoveto{\pgfpointorigin}


      \node[dtreenode,initial above,initial text={}] at (0,0) (l0)  {
        jetty.util.security.\\Credential.stringEquals\_bblock\_106};
      \node[dtreenode,below=of l0] (l2)
       {jetty.util.security.\\Credential.stringEquals\_bblock\_106};
       \node[dtreenode,below=of l2] (l4)
        {jetty.util.security.\\Credential.stringEquals\_bblock\_106};
        \node[below=of l4] (l6) {};

        \node[dtreeleaf,bicolor={blue!60 and blue!60 and 0.99},below left=of
          l0] (l1) {};
        \node[dtreeleaf,bicolor={blue and blue and 0.99},below left=of l2]
        (l3) {};
        \node[dtreeleaf,bicolor={green and green and 0.99},below left=of
          l4] (l5) {};


        \path[->]  (l0) edge  node [left,pos=0.4] {$ = min(1,y) ~~$} (l1);
        \path  (l0) edge  node [right, pos=0.4] {$~~ \neq min(1,y) $} (l2);
        \path  (l2) edge  node [left] {$ = min(2,y) ~~$} (l3);
        \path  (l2) edge  node [right] {$~~ \neq min(2,y) $} (l4);
        \path  (l4) edge  node [left] {$ = min(3,y) ~~$} (l5);
        \path  (l4) edge[dotted]  node [right] {$~~ \neq min(3,y)$} (l6);
    \end{tikzpicture}
  }
  \hfill
  \caption{
  %
    (a) Jetty timing functions for local observations.
        A remote observer tries to guess the secret in green function.
      %
    (b) Jetty (local) timing functions are clustered to $20$ groups using $L_1$-norm.
        A remote observer uses the first derivatives
        and recognizes the light blue cluster as the closet
        local observation to the remote green observation.
    %
    (c) Learned decision tree model. Number of calls to basic block at
    	line 106 of stringEquals discriminates different classes of observations. }
  % \label{fig:Jetty-initial}
  \label{fig:Jetty-clustered}
  \label{fig:jetty-remote-1}
	\label{fig:jetty-remote-2}
  \label{fig:Jetty-DT}
  \vspace{-1.0em}
\end{figure*}

